Math Blind: Failures in Diagram Understanding Undermine Reasoning in MLLMs

Diagrams represent a form of visual language that encodes abstract concepts and relationships through structured symbols and their spatial arrangements. Unlike natural images, they are inherently symbolic, and entirely artificial. They thus pose unique challenges for Multimodal Large Language Models (MLLMs) distinct from natural image processing. Recent studies have shown that MLLMs often exhibit flawed reasoning and hallucinations when handling diagram inputs. We investigate here whether these limitations stem from shortcomings in the models' ability to interpret diagrams themselves. To this end, we develop a diagnostic test suite that isolates perception from reasoning. Our systematic evaluation reveals that MLLMs perform poorly on basic perceptual tasks, e.g., shape classification, object counting, relationship identification, and object grounding, with near-zero accuracy on fine-grained grounding. Further analysis shows that weak diagram perception leads to "blind faith in text", where models rely on textual shortcuts rather than visual understanding (that is, they are Math Blind). We hypothesize that enabling models to capture the inherent structural properties of diagrams, represented as graphs of primitives and their interrelationships, is essential for improving diagram understanding. Experiments with 7B and 32B MLLMs validate this assumption, with models trained on such representations achieving a +79% gain on the grounding task. Crucially, these gains transfer to reasoning, achieving 3-4% cross-suite improvements on three public benchmarks even without additional chain-of-thought reasoning data. Our findings demonstrate that low-level perception supports faithful high-level reasoning in mathematical MLLMs. We provide both methodological frameworks and empirical evidence to guide future research in this direction.

==> macro.tex <==
\usepackage{natbib}
% Standard package includes
% \usepackage{times}
\usepackage{latexsym}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets
\usepackage{url}
\usepackage{amssymb}
\usepackage[utf8]{inputenc}
\usepackage{microtype}
\usepackage{booktabs}
\usepackage{pifont} 
\usepackage{multirow}
\usepackage{makecell}
\usepackage{paralist}
\usepackage{xspace}
\usepackage{color}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{adjustbox}
\usepackage{hyperref} 
\usepackage[edges]{forest}
\usepackage{tikz} 
% \usepackage{longtable} % For tables that can span multiple pages
\usepackage{caption}
\usepackage{amsfonts}

\hypersetup{
    colorlinks,
    linkcolor={blue!80!black},
    citecolor={blue!80!black},
    % urlcolor={brown!50!black}
}
\tikzset{
    root/.style =             {align=center, text width=1cm, rounded corners=3pt, line width=0.3mm, fill=gray!10, draw=gray!80, font=\small},
    % demographic 
    demographic/.style =         {align=center, text width=1.8cm, rounded corners=3pt, line width=0.3mm, fill=blue!10, draw=blue!80, font=\footnotesize},
    demographic_work/.style =    {align=center, text width=10cm, rounded corners=3pt, line width=0.3mm, fill=blue!10, draw=blue!0, font=\footnotesize},
    % character 
    character/.style =         {align=center, text width=1.8cm, rounded corners=3pt, line width=0.3mm, fill=red!10, draw=red!80, font=\footnotesize},
    character_work/.style =    {align=center, text width=10cm, rounded corners=3pt, line width=0.3mm, fill=red!10, draw=red!0, font=\footnotesize},
    % Personalization
    personalization/.style =           {align=center, text width=1.8cm, rounded corners=3pt, line width=0.3mm, fill=cyan!10, draw=cyan!80, font=\footnotesize},
    personalization_work/.style =      {align=center, text width=10cm, rounded corners=3pt, line width=0.3mm, fill=cyan!10, draw=cyan!0, font=\footnotesize},
    % risks
    risk/.style =         {align=center, text width=1.8cm, rounded corners=3pt, line width=0.3mm, fill=orange!10, draw=orange!80, font=\footnotesize},
    risk_work/.style =    {align=center, text width=10cm, rounded corners=3pt, line width=0.3mm, fill=orange!10, draw=orange!0, font=\footnotesize},
}


% ----------------------------------------------------
% 导言区：加载宏包并定义 remark 环境
% ----------------------------------------------------

% ----------------------------------------------------
% 导言区
% ----------------------------------------------------



% If the title and author information does not fit in the area allocated, uncomment the following
%
% \setlength\titlebox{7cm}
%
% and set <dim> to something 5cm or larger.
\newcommand{\new}[1]{\textcolor{purple}{{#1}}}
\newcommand{\todo}[1]{\textcolor{red}{{[$\blacksquare$ TODO: #1]}}}
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\wo}{\textit{w/o}\xspace}
\newcommand{\dq}[1]{``#1''}
\newcommand{\sq}[1]{`#1'}
\newcommand{\cjj}[1]{\textcolor{blue}{{[cjj: #1]}}}
\newcommand{\jj}[1]{\textcolor{cyan}{\small{\bf [JJ: #1]}}}
\newcommand{\zheng}[1]{\textcolor{brown}{{[zheng: #1]}}}
\newcommand{\zhouh}[1]{\textcolor{red}{\bf \small [#1 --zhouh]}}
\newcommand{\yuxuan}[1]{\textcolor{red}{[Yuxuan: #1]}}



\newcommand{\etc}{\textit{etc}\xspace}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\customcite}[2]{\hyperlink{cite.#2}{#1}}

% \setlength\tabcolsep{3.5pt}

\newcommand\footnoteplain[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\usepackage{CJK}
% \pagestyle{plain} % very strange, fixes page number centering problem.



==> sec/0_abs.tex <==

% \begin{center}
% \begin{minipage}{0.5\textwidth}

\begin{abstract}

Diagrams are a form of visual language, representing complex concepts and their interrelationships through structured symbols, shapes, and spatial arrangements. Unlike natural images, they are inherently symbolic and abstract.  Diagrams thus pose significant challenges for Multimodal Large Language Models (MLLMs) that are typically trained on large numbers of images. Current benchmarks conflate perceptual and reasoning tasks, making it difficult to assess whether MLLMs genuinely understand mathematical diagrams beyond superficial pattern recognition and textual memorization. %beyond superficial pattern recognition. %failures originate from visual misinterpretation or reasoning limitations. 
To address this gap, we introduce \ourMethod, a benchmark specifically designed to isolate and evaluate diagram perception in MLLMs. \ourMethod~comprises 1.2K diagrams and 1.6K carefully curated questions spanning four perception tasks: shape classification, object counting, relationship identification, and object grounding, covering diverse domains including plane geometry, solid geometry, and graphical representations. Our evaluation of MLLMs reveals that their ability to understand diagrams is limited, particularly in fine-grained grounding tasks. In response, we construct the perception-oriented \ourdata, a 200K dataset that represents geometric diagrams as structured graphs capturing primitives, their spatial relationships, and fine-grained bounding boxes. Training MLLMs on \ourdata leads to significant gains in perceptual accuracy, which in turn substantially improves mathematical reasoning. Our benchmark and dataset establish critical standards for evaluating and advancing multimodal mathematical understanding, providing valuable resources and insights to foster future MLLM research. All implementations will be released upon acceptance. 
\end{abstract}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Computer vision has traditionally focused on image-based perception tasks such as object detection~\cite{meng2021conditional,zhu2020deformable}, segmentation~\cite{li2021ctnet,mishra2019ocr}, and spatial reasoning~\cite{cheng2025spatialrgpt,driess2023palm,lin2014coco}. These capabilities form the foundation for higher-level visual reasoning in recent advances in Multimodal Large Language Models (MLLMs)~\cite{achiam2023gpt,llava,sun2024arcana}.  Despite remarkable successes in general vision tasks, current MLLMs face considerable challenges in interpreting mathematical diagrams. 
%The idea that the vertices of a quadrilateral might lie on a circle, or the conditions that render two triangles similar, are hard to learn in pixel coordinates.

Although both natural images and symbolic diagrams can be represented as grids of pixels, they constitute very different forms of information.  Images represent samples of the intensity of the real world. Diagrams, despite taking many forms,  are uniformly generated by humans as abstract visual representations of concepts characterized by precise geometric structures and symbolic notations~\cite{lumathvista,zhang2024mathverse}. Images are thus natural collections of signals, where diagrams are artificial collections of symbols.
%These diagrams provide a unique perceptual challenge: the explicit structural constraints require genuine visual interpretation rather than pattern recognition or textual heuristics, positioning them as an essential benchmark for evaluating the true visual perception capabilities of multimodal models. 
%Diagrams are pervasive across educational contexts, scientific communication, and problem-solving in STEM disciplines. 
Diagrams are critical to human visual communication across educational contexts, scientific discourse, and STEM problem-solving, but the problem of analyzing symbolic visual information is far broader. 

% Diagrams are critical to many forms of human visual communication, but the problem of analyzing symbolic visual information constructed by humans is far broader. Images of buildings, farms, suburbs and crowds exhibit similar visual language and interpreting them thus represents a similar challenge.  It is also a challenge that similarly remains unsolved.
% Developing models capable of understanding symbolic information in diagrams is a critical milestone in advancing visual machine intelligence~\cite{Cromley2010,deRijke1999}.  
%Such diagrams are pervasive across educational contexts, scientific communication, and problem-solving in STEM disciplines, making the ability to process them accurately a critical milestone for multimodal understanding. 
% Moreover, mathematical diagrams provide a unique perceptual challenge: their explicit structural constraints require genuine visual interpretation rather than pattern recognition or textual heuristics, positioning them as an essential benchmark for evaluating the true visual perception capabilities of multimodal models.

Recent benchmarks such as MathVista~\cite{lumathvista} and
MathVerse~\cite{zhang2024mathverse} evaluate mathematical visual reasoning in MLLMs. These works conflate perception with reasoning, however, 
because they assess performance on complex  
tasks that combine diagram interpretation and mathematical reasoning.  It thus remains unclear whether the performance truly reflects the models' ability to comprehensively understand the symbolic information in diagrams.
%%A reveals a stark contrast: while humans can solve fundamental perception tasks ``at a glance'', 
% Consequently, they fail to reveal whether model errors originate from perceptual misinterpretations or reasoning inadequacies. 
Perceptual misinterpretations propagate downstream, leading to faulty reasoning and frequent hallucinations, although the final answer may occasionally still be correct ~\cite{bai2024hallucination,jiang2024hallucination,wang2024mllm}. 
% This conflation of perception and reasoning raises a fundamental question: do MLLMs genuinely perceive mathematical diagrams, or do they rely predominantly on superficial pattern recognition?
Developing models capable of understanding symbolic information in diagrams is a critical milestone in advancing machine intelligence~\cite{Cromley2010,deRijke1999}. 

\begin{wrapfigure}{r}{6.5cm}
\centering
\vspace{-0.5cm}
\includegraphics[width=.45\textwidth]{img/radar_fig1.pdf} 
\caption{Performance on \ourMethod\ reveals that diagram interpretation is challenging for MLLMs, particularly in fine-grained grounding tasks. \basemathplus-7B, trained on \ourdata, significantly outperforms comparators.}
\label{fig:intro1}
\vspace{-1.8em}
\end{wrapfigure}

Motivated by the above we have designed a benchmark to isolate and rigorously evaluate mathematical perception in MLLMs. \ourMethod~features problems that humans can solve ``at a glance'' without extensive reasoning. The benchmark contains 1,198 images and 1,609 carefully designed perception-oriented questions across four distinct task categories: shape classification, object counting, relationship identification, and object grounding. These tasks span three core mathematical domains—plane geometry, solid geometry, and graphical representations (line, bar, and pie graphs)—and question formats (multiple-choice, true/false, and free-form).

%encompass various difficulty levels and 
% \vspace{-.5em}

We systematically evaluate current MLLMs on \ourMethod\ to investigate key questions:

%(both open-source and proprietary) 
\textbf{\textit{1. Do current MLLMs genuinely perceive mathematical diagrams? }}  Fig.~\ref{fig:intro1} presents the performance of eight current MLLMs—six generic models and two math-specific models—across four perception-focused tasks in \ourMethod\ (see Tab.~\ref{tab:main_results} for more MLLM results). Among the generic MLLMs, Qwen2.5-VL-7B \cite{bai2025qwen2.5} achieves the highest average accuracy, followed by GPT-4o. But both suffer from severe hallucinations—responding to simple questions with unnecessarily long chains-of-thought and generating irrelevant visual content (see Fig.~\ref{fig:erro}). The math-specific \basemath ~\cite{svemath}, with a geometric primitive visual encoder, performs on par with Qwen2.5-VL-7B in shape classification and relationship identification. However, all models, including Qwen2.5-VL-7B and DeepSeek-VL2-Small, which are trained on nearly 2T natural images, consistently underperform on fine-grained bounding box grounding, with accuracy below 20\%.


We developed \ourdata, a geometric perception-oriented dataset in both image-caption and instructive formats, to address the shortcomings of existing datasets. In contrast to existing image-caption-based visual training datasets (such as MAVIS \cite{zhang2024mavis}, and AutoGeo \cite{huang2024autogeo}, two of the largest in math vision), \ourdata\ provides explicit structured information, including shapes, attributes, locations, and relationships (see Fig.~\ref{fig:intro_subfig1}). 

To demonstrate the value of \ourdata we train a \basemathplus model which is an improved version of \basemath.  We first train only the vision-language projector using the image-caption data. In the second self-fine-tuning (SFT) stage, the instructive conversational data is used to jointly update the visual encoder, the projector, and the large language model. The resulting model achieves the highest performance among both generic and math-specific models, particularly excelling in grounding tasks with a +79\% improvement. Additional results for Qwen2.5-VL-7B/32B trained with \ourdata\ are provided in \S\ref{exp:mainresults}.


% Given that humans easily solve perception tasks ''at a glance'' with minimal cognitive effort, we explore the internal structure of MLLMs by isolating perception capabilities from reasoning. Specifically, by freezing the language model component and training only the vision-language projector module of \basemath\ on our newly curated geometric dataset \ourdata, we demonstrate substantial improvements in perceptual performance, indicating that the projector largely determines the perceptual abilities of MLLMs (refer to Table \ref{tab:compare_sft}).

% If the model relies only on pattern recognition without truly perceiving the image, it risks incorrect answers due to the image’s explicit structural constraints.  thereby clearly differentiating perception from reasoning processes. 
% Through controlled experiments, we demonstrate that geometric perception is particularly sensitive to several factors, including the number of objects, visual quality, visual and textual distractors, and Chain-of-Thought (CoT) reasoning strategies. Figure \ref{fig:intro1} reveals notable vulnerabilities of MLLMs: a) Increased the number of objects reduces accuracy: adding multiple objects in a single image negatively impacts classification, counting, and bounding box grounding; b) Visual distractors impair perception: While Gaussian noise has a minor effect, foreground scribbles and auxiliary lines significantly disrupt recognition; c) Textual distractors affect visual processing: irrelevant textual details (\eg, figure style, line colors, background attributes) negatively impact object relationship identification; d) CoT interferes with perception tasks: Although CoT improves reasoning, it disrupts perception-focused tasks that require minimal reasoning, particularly in Qwen-series models and GPT-4o (Figure \ref{fig:erro}).


\textbf{\textit{2. Does stronger perceptual ability lead to better reasoning performance?}} Our findings reveal that accurate diagram perception leads to more faithful reasoning steps. Regarding perception ability, as shown in Fig.~\ref{fig:intro_subfig2} (marked with colored dot points), training with our proposed 100K alignment dataset significantly improves perception performance compared to 100K AutoGeo and 588K MAVIS (by 23.0\% and 35.6\%, respectively). In contrast, the other two variants perform worse than the baseline (\basemath-7B), particularly with MAVIS diagram-caption pairs, due to high uncertainty and out-of-distribution nature of real-world geometric diagrams.

% We attribute the low perception ability of models trained with MAVIS diagram-caption pairs to the high uncertainty and out-of-distribution nature of real-world geometric diagrams.


To further investigate its effect on reasoning ability, we continue fine-tuning each model using the same reasoning training dataset (MathV360K~\cite{shi2024math-llava}) and our 100K instruction-style perception samples for a fair comparison.
% and Geo170K-SFT \cite{gao2023gllava}
Our model achieves 28.1\% accuracy on the MathVista reasoning benchmark—an improvement of +$\sim$4\% over others. This gain is non-trivial, considering that Multi-Math-7B \cite{peng2024multimath}, trained on 600K samples with additional reinforcement learning, achieves only 26.9\% accuracy. Our model accurately identifies relevant visual elements, enabling it to generate more valid and faithful reasoning steps (see model responses in Figs.~\ref{fig:response}/\ref{suppfig:response_appendix_1}-\ref{suppfig:response_appendix_3}).


In summary, our contributions are as follows:
\begin{itemize} \setlength\itemsep{0em}
\item We introduce \ourMethod, a benchmark for evaluating diagram perception in geometry and graphical domains. \ourMethod~isolates perception capabilities through carefully designed tasks, with data quality ensured through rigorous human verification.

\item We systematically investigate how perception influences mathematical reasoning and quantitatively analyze factors that affect MLLMs' perceptual capabilities (see \S\ref{exp:abla}). Ablation results reveal a prevalent ``blind faith in text'' phenomenon, leading models to overly rely on the available text  when conflicts arise between images and text.

\item We construct \ourdata, a geomatic perception-oriented dataset comprising 200K high-quality \{geometry-image, text\} pairs (100K diagram-caption and 100K conversation) that explicitly structure diagrams into shapes, attributes, locations, and relationships. By offering precise grounding cues and minimizing ambiguity, \ourdata\ enhances MLLMs’ visual perception and reasoning performance.
\end{itemize}

% We envision \ourMethod\ as a valuable testbed to bridge the gap between low-level visual perception and high-level mathematical reasoning, ultimately facilitating the development of more robust and reliable multimodal models for mathematical understanding.

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.66\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/Intro_Demo.pdf}
   \caption{}
        \label{fig:intro_subfig1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/daxiao_point_nips.pdf}
    \caption{}
    \label{fig:intro_subfig2}
\end{subfigure}
% \vspace{-1.em}
 \caption{Illustration of diagram-caption alignment training datasets, \textit{w.r.t.}, AutoGeo, MAVIS, and our proposed \ourdata (Fig. \ref{fig:intro_subfig1}). Fig.~\ref{fig:intro_subfig2} demonstrates a positive correlation between low-level perception and high-level reasoning tasks, evaluated on \ourMethod\ and MathVerse. Clear diagram perception leads to substantial improvements in mathematical reasoning performance.}
\vspace{-1.2em}
\end{figure*}
% we discover a `blind faith in text' phenomenon: VLMs disproportionately trust textual data over visual data when inconsistencies arise, leading to significant performance drops under corrupted text and raising safety concerns.
% % Computer vision was designed to enable machines to interpret images like human vision[]. Early efforts focused on extracting meaningful information from images, forming the basis of perception—the foundation for higher-level reasoning and decision-making. Accurate perception of objects, attributes, and spatial relationships is essential for scene analysis, relationship inference, and advanced computer vision tasks []. Yet in the modern era of large language models (LLMs), research has shifted from core perceptual tasks to vision-language tasks, primarily expressed in natural language, which emphasize the ability to reason over visual and textual information.% rather than directly enhancing visual perception.

% Computer vision was originally developed to enable machines to interpret images similarly to human vision. Early research emphasized fundamental perception tasks~\cite{driess2023palm,lin2014coco}, \ie, object detection~\cite{meng2021conditional,zhu2020deformable}, segmentation~\cite{li2021ctnet,mishra2019ocr}, and spatial reasoning~\cite{cheng2025spatialrgpt}, establishing the foundation for  higher-level reasoning and decision-making.  However, in the era of Multi-modal Large Language Models (MLLMs)~\cite{achiam2023gpt,llava,sun2024arcana}, the focus has shifted to vision-language tasks, where models primarily process visual information through natural language interactions rather than direct visual perception. 

% Early MLLMs~\cite{llava,xiao2023florence} focused on Visual Question Answering (VQA)~\cite{goyal2017vqav2,scienceQA}, requiring holistic image understanding. Recently, fine-grained visual perception, linking textual descriptions to specific image regions, has gained attention for improving model interpretability and enabling a more structured analysis of visual content~\cite{youferret,groma}. Those advancements enable MLLMs to tackle tasks requiring detailed visual comprehension, marking significant progress in fine-grained natural image understanding.

% The ability to accurately process mathematical diagrams represents a critical frontier for MLLMs, as these visual representations are central to education, scientific communication, and problem-solving across STEM disciplines. Beyond their practical importance, mathematical diagrams offer a distinctive test case for visual perception: they contain precise structural constraints with specific notational conventions that must be correctly interpreted before any reasoning can occur. This positions mathematical diagram perception as an ideal domain for investigating whether MLLMs truly "see" or merely recognize patterns in visual inputs.

% % For instance, grounding associates textual descriptions with specific image regions, ensuring region-level alignment, which is crucial for high-level semantic reasoning in MLLMs. Without proper alignment, models may hallucinate, producing unrelated or illogical responses disconnected from the image []. 
% %Intuitively, if a model fails to interpret a diagram correctly, it cannot effectively leverage visual cues to support reasoning. 
% % Thus, Ferret~\cite{youferret} integrates the grounding abilities and unlock the referential ability in dialogue. This advancement enables MLLMs to tackle tasks requiring detailed visual comprehension, marking significant progress in fine-grained natural image understanding.


% Despite the remarkable advancements of current MLLMs~\cite{wang2023cogvlm,llava,wu2024deepseekvl2}, accurately identifying mathematical primitives remains underexplored. Math diagrams present significant semantic gaps from general visual scenarios due to their abstract curves, shapes, and symbols within a monochromatic color scheme. Thus, existing MLLMs struggle to interpret diagrams effectively, often relying on textual shortcuts rather than genuine diagram comprehension ~\cite{lumathvista,zhang2024mathverse,zhou2024mathscape}. However, mathematical images provide critical structural constraints, encoding spatial, proportional, and relational information, which is essential for complex problem-solving.  MathVista~\cite{lumathvista} and MathVerse~\cite{zhang2024mathverse} aim to evaluate mathematical visual reasoning but conflate perception and reasoning by including numeric calculations and proof generation, obscuring whether failures stem from reasoning limitations or misperception.

% Visual perception errors lead to incorrect reasoning, causing models to hallucinate non-existent information, highlighting the need for perceptual enhancement in MLLMs~\cite{bai2024hallucination,wang2024mllm,jiang2024hallucination}. To systematically assess MLLMs' mathematical primitive perception abilities, we propose \ourMethod, a novel benchmark for evaluating mathematical perception-demanding skills in MLLMs, spanning coarse-to-fine tasks, \eg, shape classification, object counting, spatial and mathematical relationships, and bounding box localization. \ourMethod\ consists of 1.2K images and 2.6K questions, categorized by difficulty (easy, medium, hard) and structured across three key domains—plane geometry, solid geometry, and graphs—evaluated through multiple-choice, true/false, and free-form answers.
% %Consequently, their evaluations rely primarily on top-1 accuracy of textual reasoning answers, failing to isolate and measure fundamental perceptual abilities. 
% %Thus, given the same visual encoder, larger-scale LLMs generally boost mathematical MLLM performance.

% %as performance is primarily measured by top-1 accuracy of answers,
% % rather than direct perception metrics. For example, evaluation samples are designed to prevent models from solving problems via text alone, yet they fail to quantify fundamental perception errors and do not offer structured feedback on classic computer vision perception tasks. Moreover, these benchmarks still incorporate elements such as numeric calculations and proof generation, which do not isolate the perception challenges.

% % To address this gap, we propose a systematic exploration of visual perception in mathematical diagrams, focusing on geometric perception—the ability to recognize basic geometric shapes, spatial relationships, and mathematical constraints (\eg, perpendicularity, parallelism, and incircle relationships). These low-level perception abilities are essential building blocks for higher-order mathematical reasoning and problem-solving.


% By assessing the perception capabilities of current MLLMs, we investigate three critical research questions:
 
% \begin{enumerate}
% \item \textbf{\textit{What factors influence MLLMs' geometric perception?}}
% To systematically investigate this, we examine five key factors that contribute to mathematical perception challenges in \ourMethod: the number of objects, object quality, visual distractors, text distractors, and Chain-of-Thought (COT) responses. Through controlled experiments on five state-of-the-art MLLMs, we uncover the following findings: a) Increased the number of objects reduces accuracy: adding multiple objects in a single image negatively impacts classification, counting, and bounding box grounding (\%, \%, \%); b) Visual distractors impair perception: While Gaussian noise has a minor effect, foreground scribbles and auxiliary lines significantly disrupt recognition; c) Textual distractors affect visual processing: irrelevant textual details (\eg, figure style, line colors, background attributes) negatively impact object relationship identification; d) CoT interferes with perception tasks: Although CoT improves reasoning, it disrupts perception-focused tasks that require minimal reasoning, accounting for 70\% of perception errors.




% % We systematically exam the underlying factors that lead to mathmadical perception challenges on \ourMethod. We quantitatively study five state-of-the-art MLLMs perceptual sensitivity to numbers of objects, object qulatiy, visaul distrctors, text distractors, and CoT interfere. Our controlled experiments yield the following findings regarding MLLMs’ primitive perception: a) increasing the number of obeject from one would decrease both classdication/couning, espically  the  bounding box groundong (\%,\% and \%). 2) incorporating Gaussian noise  silght decrease the percepual ablity compared with visaul distrctors such as drawting scrible and auxliary lines in forground obejcts. 3) priving the unrealted textual dicrption \wrt question could interfer the visual perception and negtively affcte the perforamce. for example, we ask the task of relationships among obejcts, and we provide the figure style information, color of line/foregorunf and backdound. 4)  While existing studies primarily focus on the performance improvements CoT brings to reasoning tasks, they often overlook whether CoT could inadvertently disrupt the model’s ability to solve perception tasks that require minimal reasoning, counting 70\% for perception erros.
% %\( \sim  \mathcal{N}(\mathbf{0}, \mathbf{0.3}) \) higher than acertain variaance of Gaussian noise does not affect MLLMs’ performance, and this threshold seems to align well with human perception.


% % b. Does CoT interfere with perception tasks? yes

% % \item \textbf{\textit {Is it necessary to  modify the reasoning process for perception improvement?}} 
% \item \textbf{\textit{Which module predominantly determines the perceptual ability of MLLMs?}}
% Since perception requires minimal or no reasoning and can be solved by humans `at a glance', we investigate its dependence on model components by freezing the LLM and training only the projector layer, which aligns visual and language spaces for visual understanding. Training \basemath\ on our 300K synthetic alignment dataset (\ourdata), covering shapes, relationships, and box-level instruction-following data (see Section  for details), significantly improves performance across all tasks, achieving a 53\% average accuracy gain.


% %by usning our sythetic dataset, specificlly designed for perception task (see section for more details).  without modifying reasoning of LLM, the viusal perception increase a lot (vs. ). 

% % d. Dose better perception assit the reasoing ablity? yes

% \item \textbf{\textit{What type of alignment dataset enhances perception and supports reasoning?}}
% To investigate this, we utilize different mathematical visual datasets (MAVIS, AutoGeo, and \ourdata) for first-stage feature alignment training, followed by a consistent instruction dataset for second-stage self-finetuning. As shown in Figure X, datasets with less ambiguity/complexity and explicit instruction significantly enhance both perception and reasoning. For instance, \basemath+\ourdata, achieving 70\% perception accuracy, reaches 26\% reasoning accuracy, surpassing models trained on other mathematical alignment datasets by +6.8\% in both perception and reasoning. Moreover, our findings highlight a strong positive correlation between fine-grained visual perception and reasoning performance. When models accurately identify relevant visual elements, they generate valid and faithful reasoning steps with fewer hallucinations (see model response).

% % Intuitively, a `blind' VLM that lacks proper visual grounding tends to answer based on LLM priors, often producing responses that are unrelated to the diagram.

% \end{enumerate}

% %Through our systematic evaluation, we find that perception-demanding tasks pose significant challenges for current MLLMs. MATHGLANCE synthesizes plane geometric diagrams, reformats CLEVR for solid geometry, and integrates FigureQA for graphical reasoning (e.g., line/bar/pie charts), comprising 3,807 questions across multiple-choice, true/false, and free-form formats (see Section X for data distribution). While humans achieve an average accuracy of 96.73%, MATHGLANCE proves highly challenging for existing multimodal LLMs: even GPT-4o and DeepSeek-VL2-Small achieve only 51.26% and 45.72% accuracy, merely 13.17% and 7.63% above random guessing. These results highlight that perceptual abilities in mathematical MLLMs have been largely overlooked. Moreover, our findings suggest that stronger perception capabilities could enhance reasoning performance.




% In summary, our contributions are as follows:
% \begin{itemize} \setlength\itemsep{0em}
% \item We emphasize the significance of fine-grained geometric perception and introduce \ourMethod, a benchmark covering a comprehensive range of mathematical diagrams, including plane and solid geometry as well as line, dot, bar, and pie graphs. The dataset undergoes rigorous human verification to ensure high-quality evaluation for the community.

% \item We are the first to systematically investigate the extent to which perception enhances mathematical reasoning. Our controlled experiments quantitatively analyze MLLMs' perceptual sensitivity to factors. 

% %We find that failing to perceive mathematical elements leads to hallucinations**, where models generate **illogical CoT for tasks solvable by humans at a glance**.

% \item We construct \ourdata, a \textbf{Geo}matic \textbf{Pe}rce\textbf{P}tion-oriented dataset comprising 300K high-quality geometry image-text pairs. Unlike existing diagram-caption datasets, which ambiguously merge descriptive elements, \ourdata decomposes diagrams into explicit object shapes, attributes, relationships, and locations, enhancing clarity and instructiveness. \ourdata significantly improves MLLMs' perceptual capabilities, which in turn enhances their reasoning abilities.
% \end{itemize}

% We believe \ourMethod\ serves as an effective testbed for bridging the gap between low-level perception and high-level reasoning in MLLMs, fostering advancements in mathematical visual understanding.

% % Our controlled experiments yield the following findings regarding MLLMs' visual perception performance:

% % We quantitatively study MLLMs’ perceptual sensitivity to relative object sizes and iden- tify various visual factors that contribute to this sensitiv- ity. 

% % and conduct controlled intervention studies to measure the ef- fect of each factor on MLLMs’ perception


% % 4. This paper aims to highlight crucial aspects of visual perception that have been overlooked when evaluating multimodal LLMs. 

% % 4. to what extent and how much CoT reasoning can benefit multimodal challenges still remains an open question.  MAVIS (synthesis part) (Zhang et al., 2024) and Geom- Verse (Kazemi et al., 2023) at the same data scale for a fair comparison. Specifically, we sample the data from each dataset to different scales.


% %autogeo: Firstly, draw a Rectangle ABCD, creating a semicircle outside with CD as the diameter, and then eliminate the side CD..  
% %each shape is connected to its parent shape via a single side or a single (vertical) angle.  Unlike previous-generation engines, which primarily focus on constructing geometric images through the combination of polygons or circles.  synthetic or abstract geometric constructions that do not typically occur in real-world geometric scenarios. In contrast, the right set illustrates geometric cases that are commonly encountered in real-world applications, adhering to practical constraints and natural geometric properties.

% %These figures often include unnatural or arbitrary compositions of shapes, such as irregularly connected polygons, disconnected circular arcs, or structurally unsupported configurations that lack clear geometric or physical relevance. In contrast, the right set illustrates geometric cases commonly found in real-world applications, adhering to fundamental geometric properties, such as symmetry, congruence, parallelism, and perpendicularity. These cases are often encountered in engineering, architecture, and mathematical problem-solving, making them more representative of practical geometric reasoning


 


==> sec/3_method.tex <==
\section{\ourMethod}
% \vspace{-.5em}
% Our goal is to systematically evaluate the visual perception capabilities of existing Multimodal Large Language Models (MLLMs) in mathematical contexts. We aim to analyze the perceptual limitations of current mathematical MLLMs in tasks that humans can solve `at a glance', providing insights into the extent to which diagram perception can support complex mathematical reasoning. \textbf{\textit{Current MLLMs are ``blind'' to diagram understanding, yet they should be capable of both seeing and reasoning like humans.}}

% \textbf{\textit{Current MLLMs are `blind' yet expected to see and reason similar to humans.}}

This section first introduces \ourMethod\ (\S \ref{main:overview}) with a data distribution analysis. We then describe the synthetic construction process for plane geometry, as well as the reformatted CLEVR \cite{johnson2017clevr} and FigureQA \cite{kahou2017figureqa} datasets for solid geometry and graphs in \S\ref{main:bechmark}. Finally, we introduce the perception-oriented \ourdata, and highlight its unique characteristics in comparison to existing mathematical visual alignment training datasets (\S\ref{main:geodet}).

\subsection{Overview}
\label{main:overview}
Existing mathematical visual reasoning benchmarks often conflate perception with higher-level tasks such as numerical calculation and proof generation. As evaluation is based solely on final answers, intermediate perception errors remain undetected. Thus, it remains unclear whether MLLMs genuinely perceive diagrams or merely rely on the prior knowledge of powerful LLMs. We introduce \ourMethod, a novel benchmark designed to evaluate MLLMs' perception-demanding abilities through both quantitative and qualitative analysis across coarse-to-fine granularity levels.
% Existing mathematical visual reasoning benchmarks often conflate perception with higher-level reasoning tasks, such as numeric calculations and proof generation. We introduce \ourMethod, a novel benchmark designed to evaluate MLLMs' mathematical perception-demanding abilities through both quantitative and qualitative analysis across coarse-to-fine granularity levels. 

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth, trim=0 0 0 20, clip]{img/planGeo-Q-A.pdf} 
\vspace{-0.5 cm}
\caption{Sampled \ourMethod~ examples from plane geometry \textit{w.r.t.} each question-answer (Q\&A) type, covering shape classification, object counting, relationship identification, and object grounding (from left to right). The green dotted bounding boxe is shown for illustration purposes only and are not provided as input to the models.}
\label{fig:planedemo}
\vspace{-1em}
\end{figure*}

\noindent \textbf{Data Composition.} To comprehensively assess the perceptual abilities of MLLMs in mathematical contexts, our evaluation images cover plane geometry (66\%), solid geometry (20\%), and graphs (14\%), including lines, bars, and pie charts. To facilitate MLLM evaluation, we formulate all tasks—except for bounding box grounding (free-form)—as multiple-choice or true/false question-answering problems. In total, we contribute 1,609 questions and 1,198 unique images, ensuring an even distribution across the different perception tasks. Detailed statistics for data composition are presented in Tab.~\ref{tab:statis} of the Appendix. 

%, all of which primarily require MLLMs to analyze the image with minimal thinking to generate answers. 
\noindent \textbf{Categorization.} The benchmark encompasses \textit{shape classification}, \textit{object counting},  \textit{relationship identification}, and \textit{object grounding}. Fig.~\ref{fig:planedemo} shows example illustrations of plane geometry (see \S\ref{supp:showdemo} for additional examples).  Key features are as follows:  
\begin{itemize} \setlength\itemsep{0em}
\item Shape classification is a classic vision task where the model identifies object classes based on attributes, \textit{i.e.}, vertices, material, color, and size. Our dataset includes a diverse set of geometric categories, comprising 16 basic shapes for plane geometry, 3 CLEVR-defined~\cite{johnson2017clevr} objects for solid geometry, and 5 graphical elements as defined in FigureQA~\cite{kahou2017figureqa}.
\item Object counting requires models to determine either the total number of objects in an image or a specific shape count, \textit{i.e.}, the number of circles or triangles present.
\item Relationship identification evaluates models' understanding of 4 spatial and over 10 mathematical relationships between pairs of geometric primitives.
\item Object grounding evaluates  fine-grained localization  by requiring MLLMs  to accurately predict the top-left and bottom-right coordinates in the format (x1, y1, x2, y2) for an object within the image. This ensures that models can precisely identify and localize geometric structures based on textual descriptions.
\end{itemize}

% \ourMethod\ is designed to enhance MLLMs' ability to process mathematical visual information by reinforcing their capacity to recognize geometric structures, quantify objects, and understand spatial relationships. Accurately identifying math-related visual elements is a foundational step toward deeper image comprehension, enabling MLLMs to bridge visual perception with symbolic reasoning. By mastering these fundamental tasks, MLLMs can develop more robust reasoning capabilities, ultimately improving their performance in vision-based mathematical problem-solving.


% Figure xx presents demo illustrations of our perception tasks in \ourMethod. Key features are as follows:  
% \begin{itemize} \setlength\itemsep{0em}
% \item Shape classification is a classic classification task in computer vision, where the model is required to identify the class name of a specific object defined along with its attributes, \ie, vertices, material, color, and size. Our dataset includes a diverse set of geometric categories, comprising 16 basic shapes for plane geometry, 3 CLEVR-defined objects for solid geometry, and 5 graphical elements as defined in FigureQA.
% \item Object counting requires models to determine either the total number of objects in an image or a specific shape count, \ie, the number of circles or triangles present.
% \item Relationship identification evaluates models' understanding of 4 spatial and 10 mathematical relationships among objects. The model is tasked with identifying the relationship between two geometric primitives. 
% \item Object grounding evaluates bounding box localization by requiring MLLMs to accurately predict the top-left and bottom-right coordinates in the format (x1, y1, x2, y2) for a specified object within an image. This ensures that models can precisely identify and localize geometric structures based on textual descriptions.
% \end{itemize}
These four tasks are designed to isolate and assess fundamental perception capabilities, distinguishing low-level visual recognition from high-level reasoning.


%  \begin{figure}[t]
% \centering
% \includegraphics[width=.25\textwidth]{img/bing.pdf} 
% \caption{Subjects and tasks distribution of \ourMethod.}
% \label{fig:bing}
% \vspace{-1em}
% \end{figure}

\subsection{Dataset Construction}
\label{main:bechmark}
\subsubsection{Synthetic Data Engine for Plane Geometry}
We design a data generation engine to synthesize geometric diagrams along with structured JSON annotations. This pipeline enables controlled shape generation, relationship modeling, and visual attribute assignment, ensuring diverse and well-balanced datasets across perception tasks. 

\noindent \textbf{Structured Annotations for Geometric Primitives.}  Fig.~\ref{fig:dataengine} describes the entire generation process. Inspired by AlphaGeometry~\cite{alphageo}, we use geometric clauses as fundamental units to construct complex plan geometric figures.  A geometric clause is a formalized description of basic geometric objects and mathematical relationships, along with their properties or attibutes, \textit{a.k.a.} prerequisite points.  We first construct two geometry substrate pools, one containing 16 different geometric shapes (\textit{i.e.}, isosceles triangle, square, rectangle, parallelogram, isosceles trapezoid, pentagon, circle $\dots$ ellipse and segment), and the other defining 10 mathematical relationships (\textit{i.e.}, on, intersection, parallel, perpendicular, tangent, $\dots$ and reflection). We then randomly sample one or more substrates from these pools and pass them through a verifier, which ensures that logically paired shapes and relationships are preserved in the construction of valid geometric images. The verifier makes decisions based on either manually designed rules, fundamental mathematical knowledge, or prerequisite points. For example, parallel lines cannot intersect, and without enough prerequisite points, an angle trisection clause is invalid.
% For example, parallel lines cannot intersect, making an intersection clause invalid. Similarly, angle trisection requires a predefined angle, which cannot be constructed without enough prerequisite points for angle consturction. 
In general, the chosen relationships are enforced by introducing additional shapes into the figure, ensuring that the specified relationships are accurately maintained and geometrically consistent throughout the construction process. We finally save the outputs as structured JSON annotations for image rendering using the Matplotlib package~\cite{matplot} and generating question-answer pairs via template-based pipelines.


\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{img/data_engine.pdf}
\vspace{-.3em}
\caption{We synthesize geometric figures by randomly sampling elements from the geometric shape pool and relationship pool, ensuring consistency through a verifier that enforces logical constraints based on manually designed rules, fundamental mathematical principles, and prerequisite points. All visual elements are structured and saved in JSON format. Images are rendered using the Matplotlib package, and corresponding Q\&A pairs are generated using a template-based pipeline.}
%The synthetic construction process for plane geometry.  
\label{fig:dataengine}
\vspace{-0.5cm}
\end{figure*}

\noindent \textbf{Image Generation.} The JSON annotations define foreground and background styles, \textit{i.e.}, colors sampled from a monochromatic palette, line width, and font size, as well as object shape information (class names),  attributes (vertices labeled with random letters),  bounding box locations, and mathematical relationships. Notably, spatial relationships are generated based on the bounding box locations of two objects (\textit{e.g.}, top-left, top-right, bottom-left, bottom-right). Similar to the image rendering process in~\cite{alphageo}, we translate geometric clauses into visual representations using Python code. This process first determines coordinates of points defined in each clause for basic shape visualization, then generates new primitives based on specified relationships. To increase task difficulty, we apply image augmentations, \textit{e.g.}, Gaussian noise, irregular scribbles, and wedge-shaped symbols for congruent angles or auxiliary lines (see Figs.~\ref{suppfig:hard} and \ref{suppfig:gaussian} in the Appendix).
% \eg, adding Gaussian noise, drawing irregular scribbles, and incorporating wedge-shaped symbols for congruent angles or auxiliary lines (see Figs. \ref{suppfig:hard} and \ref{suppfig:gaussian} in the Appendix). 

%\( \sim  \mathcal{N}(\mathbf{0}, \mathbf{0.3}) \)


\noindent \textbf{Question-Answer Generation.} Based on structured annotations, we employ a template-based pipeline to generate multiple-choice and true-false questions across four perception tasks.
%: shape classification, object counting, relationship identification, and object grounding.  
For example, in constructing Q\&A pairs for shape classification, we first randomly select an object and its associated attributes from the given figure.  We then formulate a question by filling placeholders in our carefully designed templates. For true-false questions, the ground truth answer is directly derived from the JSON annotations. For multiple-choice questions, we generate plausible distractors to challenge the model’s geometric perception, combining them with the correct answer into a set of four choices. Distractors are selected from geometric candidate pools, ranging from visually similar (\textit{e.g.}, equilateral \textit{vs.} isosceles triangles) to visually dissimilar pairs (\textit{e.g.}, equilateral triangle \textit{vs.} circle). Further details on the Q\&A generation templates are provided in Tab.~\ref{tab:templates} of the Appendix. 

\subsubsection {Reformat Dataset for Solid Geometry \& Graphs} We leverage the public datasets CLEVR~\cite{johnson2017clevr} and FigureQA~\cite{kahou2017figureqa} to construct benchmarks for solid geometry and graphs, respectively. Since their original annotation formats are incompatible with our template-based Q\&A generation pipeline, we reformat them into structured JSON, consistent with the format used in our synthetic data process. Once reformatted, we apply the same Q\&A generation strategy as used for plane geometry. See \S\ref{supp:refomatdata} for details.

After generating our synthetic data and collecting public datasets, we conduct a comprehensive review to verify answer accuracy, ensure consistency between questions and diagrams, and confirm relevance to the four perception tasks, ensuring high-quality and precise dataset annotations.

\begin{table*}[!t]\footnotesize
 \caption{Performance comparison of different MLLMs on \ourMethod\ across plane geometry, solid geometry, and graphs. \textit{cls}, \textit{cnt}, \textit{grd}, and \textit{rlat} represent different question categories: shape classification, object counting, object grounding, and relationship identification, respectively. \textit{all} indicates the overall accuracy, calculated as the ratio of correctly answered questions to the total number of questions in the benchmark, while \textbf{Avg.} denotes the average \textit{all} score across all subjects.}
 \vspace{-.5em}
 \label{tab:main_results}
 \centering
 \renewcommand\arraystretch{1.2}
 \setlength{\tabcolsep}{1.6mm}{
 \resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|c|c|ccccc|ccccc|ccccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Avg.}} & \multicolumn{5}{c|}{\textbf{Plane  Geometry}} & \multicolumn{5}{c|}{\textbf{Solid  Geometry}} & \multicolumn{5}{c}{\textbf{Graphs}} \\ \cline{4-18} 
 &&& \textit{all} & \textit{cls} & \textit{cnt} & \textit{grd} & \textit{rlat} & \textit{all} & \textit{cls} & \textit{cnt} & \textit{grd} & \textit{rlat} & \textit{all} & \textit{cls} & \textit{cnt} & \textit{grd} & \textit{rlat} \\ \hline
\rowcolor{green!15}\multicolumn{18}{l}{\textit{Open-Source Generic MLLMs}}   \\ \hline
LLaVA-v1.5~\cite{llava} & 7B & 33.3 & 29.2 & 29.0 & 39.6 & 14.2 & 37.5 & 31.6 & 43.0 & 42.3 & 0.0 & 31.3 & 39.0 & 76.8 & 35.2 & 0.0 & 39.4 \\ 
LLaVA-v1.5~\cite{llava} &13B & 35.4 & 32.8 & 29.3 & 40.4 & 23.5 & 42.0 & 35.9 & 60.5 & 38.1 & 0.0 & 35.0 & 37.6 & 63.8 & 42.6 & 0.0 & 45.5 \\  
mPLUG-Owl3~\cite{ye2024mplug-owl3} & 7B & 50.0 & 36.4 & 46.7 & 41.6 & 3.9 & 58.5 & 65.3 & 95.4 & 83.5 & 0.0 & 62.5 & 48.2 & 59.4 & 77.8 & 0.0 & 66.7 \\ 
InternLM-XComposer2~\cite{dong2024internlm} &7B & 55.6 & 35.8 & 49.4 & 48.8 & 0.0 & 47.0 & 62.9 & 90.7 & 86.6 & 0.0 & 53.8 & 54.6 & 60.9 & 94.4 & 0.0 & 78.8 \\ 
Qwen2-VL~\cite{wang2024qwen2} & 7B& 51.4 & 37.9 & 47.6 & 41.2 & 12.8 & 53.0 & 64.1 & 93.0 & 78.4 & 14.3 & 55.0 & 52.3 & 84.1 & 88.9 & 3.2 & 18.2 \\ 
Qwen2-VL~\cite{wang2024qwen2} & 72B& 59.9 & 42.4 & 51.2 & 50.8 & 17.4 & 52.0 & 71.2 & 97.7 & 84.5 & 6.4 & 77.5 & 66.1 & 76.8 & \textcolor{blue}{98.2} & \textcolor{red}{\textbf{16.1}} & 84.9 \\
Qwen2.5-VL~\cite{bai2025qwen2.5}& 7B& 59.2 & 44.0 & 56.2 & 51.3 & 18.5 & 52.0 & 68.0 & \textcolor{red}{\textbf{98.8}} & 88.7 & 0.0 & 65.0 & 65.7 & 89.9 & \textcolor{red}{\textbf{100.0}} & 3.2 & 78.8 \\ 
Qwen2.5-VL~\cite{bai2025qwen2.5}& 32B& 62.2 & 43.3 & 56.9 & 54.8 & 0.0 & 67.0 & 72.5 & \textcolor{red}{\textbf{98.8}} & \textcolor{blue}{89.7} & 1.6 & \textcolor{red}{\textbf{87.5}} & \textcolor{blue}{68.8} & 91.3 & \textcolor{red}{\textbf{100.0}} & 1.6 & \textcolor{blue}{97.0}  \\
DeepSeek-VL2-Tiny~\cite{wu2024deepseekvl2}& 3B& 32.6 & 29.5 & 45.2 & 34.4 & 4.6 & 32.0 & 39.0 & 76.7 & 32.0 & 0.0 & 37.5 & 29.4 & 39.1 & 57.4 & 0.0 & 18.2 \\ 
DeepSeek-VL2-Small~\cite{wu2024deepseekvl2}& 16B& 51.5 & 37.6 & 47.6 & 43.6 & 12.5 & 48.5 & 63.8 & \textcolor{red}{\textbf{98.8}} & 70.1 & 11.1 & 60.0 & 53.2 & 76.8 & 53.7 & \textcolor{blue}{11.3} & 81.8 \\ 
InternVL2~\cite{chen2024internvl}& 8B& 48.4 & 31.9 & 44.3 & 38.0 & 0.0 & 48.5 & 62.9 & \textcolor{red}{\textbf{98.8}} & 62.9 & 4.8 & 70.0 & 50.5 & 68.1 & 75.9 & 0.0 & 66.7 \\ 
InternVL2.5~\cite{internvl2.5}& 8B& 50.7 & 35.0 & 48.8 & 36.0 & 0.0 & 60.0 & 65.6 & \textcolor{red}{\textbf{98.8}} & 72.2 & 4.8 & 70.0 & 51.4 & 68.1 & 77.8 & 0.0 & 69.7 \\ 
InternVL2.5~\cite{internvl2.5}& 38B& 63.1 & 44.0 & 59.9 & 52.0 & 2.5 & 66.0 & \textcolor{red}{\textbf{78.8}} & \textcolor{red}{\textbf{98.8}} & \textcolor{red}{\textbf{92.8}} & \textcolor{red}{\textbf{38.1}} & 72.5 & 66.5 & \textcolor{red}{\textbf{98.6}} & 96.3 & 3.2 & 69.7 \\ \hline
\bf Qwen2.5-VL$^{\boldsymbol{+}}$ (ours) & 7B&\textcolor{blue}{72.9} & \textcolor{blue}{78.5} & \textcolor{blue}{70.7} & 79.2 & 82.6 & \textcolor{blue}{85.0} & 71.9 & \textcolor{blue}{97.9} & 86.2 & 12.9 & 70.0 & 68.2 & \textcolor{blue}{94.2} & 96.3 & 4.9 & 89.4 \\ 
\bf Qwen2.5-VL$^{\boldsymbol{+}}$ (ours) & 32B&\textcolor{red}{\textbf{74.2}} & 77.9 & \textcolor{blue}{70.7} & \textcolor{blue}{79.6} & \textcolor{red}{\textbf{84.0}} & 79.5 & \textcolor{blue}{73.8} & \textcolor{red}{\textbf{98.8}} & 86.4 & 15.0& \textcolor{blue}{85.0} & \textcolor{red}{\textbf{71.1}} & \textcolor{red}{\textbf{98.6}} & \textcolor{blue}{98.2} & 2.7 &  \textcolor{red}{\textbf{99.0}} \\ \hline
\rowcolor{green!15}\multicolumn{18}{l}{\textit{Closed-Source Generic MLLMs}}   \\ \hline
GPT-4o & -& 53.3 & 42.8 & 58.4 & 53.2 & 1.1 & 62.5 & 60.7 & 72.1 & 84.5 & 1.6 & 66.3 & 56.4 & \textcolor{blue}{92.8} & 72.2 & 1.6 & 57.6 \\ 
GPT-o1 & - & 36.5 & 15.8 & 33.2 & 11.6 & 0.0 & 14.0 & 41.4 & 75.6 & 52.6 & 0.0 & 23.8 & 52.3 & 82.6 & 81.5 & 0.0 & 39.4 \\ 
GPT-o4-mini-high & - & 48.0 & 19.1 & 29.3 & 24.4 & 0.4 & 21.5 & 64.7 & 94.2 & 79.4 & 0.0 & 66.3 & 60.1 & 95.7 & 77.8 & 0.0 & 69.7 \\  \hline
\rowcolor{green!15}\multicolumn{18}{l}{\textit{Open-Source Mathematical MLLMs}}   \\ \hline 
 Math-LLaVA~\cite{shi2024math-llava}& 13B& 40.0 & 27.9 & 34.4 & 32.4 & 0.0 & 50.5 & 44.8 & 81.4 & 55.7 & 0.0 & 27.5 & 47.3 & 78.3 & 59.3 & 0.0 & 51.5 \\ 
G-LLaVA~\cite{gao2023gllava} &7B& 30.3& 25.6 & 27.8 & 41.2 & 0.4 & 38.0 & 32.3 & 45.4 & 38.1 & 4.8 & 32.5 & 33.9 & 58.0 & 37.0 & 0.0 & 42.4 \\ 
%Math-PUMA-DeepSeek-Math-VL & 7B & 44.7 & 29.3 & 45.8 & 26.8 & 0.0 & 46.0 & 46.9 & 76.7 & 62.9 & 0.0 & 32.5 & 57.8 & 92.8 & 75.9 & 0.0 & 63.6 \\
%URSA & 8B & 42.2 & 31.8 & 39.2 & 39.2 & 0.0 & 55.0 & 40.2 & 79.1 & 41.2 & 0.0 & 28.8 & 54.6 & 82.6 & 68.5 & 0.0 & 75.8 \\
MultiMath~\cite{peng2024multimath}&7B & 42.1 & 31.2 & 44.0 & 30.4 & 1.1 & 53.0 & 46.7 & 81.4 & 53.6 & 4.7 & 33.8 & 48.6 & 79.7 & 57.4 & 3.2 & 33.8 \\ 
SVE-Math-DeepSeek~\cite{svemath} & 7B& 46.6 & 35.4 & 52.4 & 36.0 & 3.6 & 51.0 & 49.4 & 77.9 & 62.9 & 1.5 & 41.3 & 55.1 & 81.2 & 75.9 & 1.6 & 69.7 \\ \hline
\bf SVE-Math-DeepSeek$^{\boldsymbol{+}}$ (ours) & 7B& 68.4 & \textcolor{red}{\textbf{84.6}} & \textcolor{red}{\textbf{75.8}} & \textcolor{red}{\textbf{88.4}} & \textcolor{blue}{82.9} & \textcolor{red}{\textbf{97.5}} & 54.1 & 85.3 & 65.8 & \textcolor{blue}{20.3}& 45.0 & 60.7 & 85.1 & 78.4 & 1.6 & 75.7 \\ 
\hline
\end{tabular}}}
\vspace{-0.5cm}
\end{table*}

\subsection{Perception-oriented Training Dataset (\ourdata)}
\label{main:geodet}
Evaluation results on \ourMethod\ reveal that both open-source and closed-source MLLMs struggle to identify relevant visual regions in symbolic and abstract mathematical diagrams,  despite their strong performance in theoretical reasoning and numerical computation. 
% After testing current MLLMs on \ourMethod\ benchmark, we find that both open-source and closed-source models lack the ability to know where to look in mathematical diagrams.
% While humans get 96\% accuracy on average, the majority of models perform below 45\% on plane geometric diragam perception, with especially low performance in the grounding task, averaging below 15\% (see Table 1 for details). 
This contrasts with human cognitive abilities, where low-level perceptual tasks are typically solved rapidly compared to high-level reasoning tasks.  This raises an important question: why do generic MLLMs—despite being trained on large-scale visual datasets—struggle to perceive mathematical diagrams? The key reason lies in the domain gap between natural images and mathematical diagrams~\cite{lumathvista,svemath}. Unlike semantically rich natural images (bitmaps), diagrams are defined by precise geometric structures and symbolic notations (vectors).  Without superficial patterns or semantic priors to exploit, MLLMs fail to generalize~\cite{geirhos}. This underscores the need for datasets that reflect the uniquely structured, graph-like nature of diagrams.  Moreover, learning from explicit structures within the data context would reduce learning complexity and enhance the problem-solving abilities of models~\cite{han2025reasoning}.  


%To overcome such perceptual limitations, the proposed \ourdata, comprising 200K high-quality image-text pairs in both diagram-caption and instruction-conversation formats, provides detailed geometric primitive information, \eg, shapes, vertices, relationships, and fine-grained bounding box coordinates.
%enhances geometric understanding and visual grounding, ultimately benefiting complex reasoning. \ourdata, 
We thus develop a structured visual dataset—where the training corpus is built from object attributes and extends to other objects based on their relationships—to improve visual attention and mitigatel MLLMs' reliance on textual shortcuts.  
%different from previous visual alignment datasets \cite{huang2024autogeo,zhang2024mavis} that offer ambiguous expressions for geometric primitives, 
% \fcolorbox{green!60!black}{green!5}{\textcolor{green!50!black}{%
% \textbf{GeoPeP} follows a structured format: First, I count \textit{\{N\}} prominent object(s) in the image. 
% Next, object \textit{\{attrbu.$^i$\}} is a \textit{\{shape$^i$\}}, and $\cdots$. 
% Furthermore, the \textit{\{shape$^i$\}} \textit{\{attrbu.$^i$\}} is located at \textit{\{box\_cor.$^i$\}}. 
% Finally, it relates via \textit{\{rela.$^{ij}$\}} to \textit{\{shape$^j$\}} \textit{\{attrbu.$^j$\}}, and $\cdots$.}} 
In specifc, \ourdata\ follows a structured format: 
%First, I count \textit{\{N\}} prominent object(s) in the image. Next, for shape information, object \textit{\{attrbu.$^i$\}} is a \textit{\{shape$^i$\}}, and $\cdots$. Furthermore, I also know the fine-grained bounding box coordinates: the \textit{\{shape$^i$\}} \textit{\{attrbu.$^i$\}} is located at \textit{\{box\_cor.$^i$\}}, and $\cdots$. Finally, let me explain the relationships: the \textit{\{shape$^i$\}} \textit{\{attrbu.$^i$\}} \textit{\{rela.$^{ij}$\}} to the \textit{\{shape$^j$\}} \textit{\{attrbu.$^j$\}}, and $\cdots$. 
\colorbox{gray!10}{%
  \parbox{\dimexpr\linewidth-2\fboxsep}{%
    {%
      First, I count \textit{\{N\}} prominent object(s) in the image. 
      Next, for shape information, object \textit{\{attrbu.$^i$\}} is a \textit{\{shape$^i$\}}, and $\cdots$. 
      Furthermore, I also know the fine-grained bounding box coordinates: the \textit{\{shape$^i$\}} \textit{\{attrbu.$^i$\}} is located at \textit{\{box\_cor.$^i$\}}, and $\cdots$. 
      Finally, let me explain the relationships: the \textit{\{shape$^i$\}} \textit{\{attrbu.$^i$\}} \textit{\{rela.$^{ij}$\}} to the \textit{\{shape$^j$\}} \textit{\{attrbu.$^j$\}}, and $\cdots$.
    }
  }
}
To further enhance the model's ability to follow instructions, we construct a task-specific instruction dataset in a multi-turn conversation format. Each question is tailored to a specific perception task, with answers presented either in free-form or as a selected option. For example: \textbf{Q}: What is the shape of object \{\textit{attrbu.$^i$}\}? \textbf{A}: \{\textit{shape$^i$}\}. See \S\ref{supp:geopep} in the Appendix for additional demonstrations.


% \begin{tcolorbox}[colback=gray!5, colframe=gray!10!black, boxrule=0.1pt, arc=2pt]
% First, I count {\#num.} object in the image. Next, for the shape information, object \textbf{\{attrbu.\}} is a \textbf{\{shape\}}. Furthermore, I also know the fine-grained bounding box coordinates: the \textbf{\{shape\}} \textbf{\{attrbu.\}} is located at \textbf{\{box. cor.\}}. Finally, let me explain the relationships: $\cdots$
% \end{tcolorbox}
% Moreover, we avoid generating irrelevant textual distractors in the ansers, as they negatively impact perception in MLLMs ~\cite{svemath}.

% as highlighted by ~\cite{svemath}, aligning relevant primitive viusal information \wrt the question is crucial; thus, we generate related QA pairs and remove redundant textual distractors.

Overall, \ourdata\ contributes to MLLM training by: (1) providing clear object attributes and their relationships, akin to graph nodes and edges, in training QA pairs; (2) offering fine-grained bounding box coordinates of elements, enabling models to systematically learn spatial awareness; and (3) integrating with reasoning-based CoT mathematical visual datasets during self-fine-tuning stage, allowing models to both perceive and reason accurately. 




